Nudge Attacks on Point-Cloud DNNs

The wide adaption of 3D point-cloud data in safety-critical applications such as autonomous driving makes adversarial samples a real threat. Existing adversarial attacks on point clouds achieve high success rates but modify a large number of points, which is usually difficult to do in real-life scenarios. In this paper, we explore a family of attacks that only perturb a few points of an input point cloud, and name them nudge attacks. We demonstrate that nudge attacks can successfully flip the results of modern point-cloud DNNs. We present two variants, gradient-based and decision-based, showing their effectiveness in white-box and grey-box scenarios. Our extensive experiments show nudge attacks are effective at generating both targeted and untargeted adversarial point clouds, by changing a few points or even a single point from the entire point-cloud input. We find that with a single point we can reliably thwart predictions in 12--80% of cases, whereas 10 points allow us to further increase this to 37--95%. Finally, we discuss the possible defenses against such attacks, and explore their limitations.

==> tables/defense.tex <==
\begin{table*}[h!]
    \caption{
        Nudge attack with a defense of furthest-point removal. We evaluate on DGCNN trained on the ModelNet10 dataset.
    }
    \label{tab:defense}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabular}{cc|ccc}
    \toprule
    Attack
    & Points Removed 
    & Natural Acc
    & Adv ACC
    & Success Rate
    \\ 
    \midrule
    1
    & 5
    & 
    & 
    &
    \\ 
    1
    & 10
    & 
    & 
    &
    \\ 
    1
    & 100
    & 
    & 
    &
    \\ 
    \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
\end{table*}
